Heterogeneous Graph Neural Network with Multi-view Representation Learning

Graph neural networks for heterogeneous graph embedding is to project nodes into a low-dimensional space by exploring the heterogeneity and semantics of the heterogeneous graph. However, on the one hand, most of existing heterogeneous graph embedding methods either insufficiently model the local structure under specific semantic, or neglect the heterogeneity when aggregating information from it. On the other hand, representations from multiple semantics are not comprehensively integrated to obtain versatile node embeddings. To address the problem, we propose a Heterogeneous Graph Neural Network with Multi-View Representation Learning (named MV-HetGNN) for heterogeneous graph embedding by introducing the idea of multi-view representation learning. The proposed model consists of node feature transformation, view-specific ego graph encoding and auto multi-view fusion to thoroughly learn complex structural and semantic information for generating comprehensive node representations. Extensive experiments on three real-world heterogeneous graph datasets show that the proposed MV-HetGNN model consistently outperforms all the state-of-the-art GNN baselines in various downstream tasks, e.g., node classification, node clustering, and link prediction.

==> sections/Abstract.tex <==
\begin{abstract}
Graph neural networks for heterogeneous graph embedding have achieved significant progress in effectively projecting nodes into a low-dimensional space for different downstream tasks.
% 
{\color{blue}However, existing works fail to fully explore the heterogeneity and semantics in the complex local structures in heterogeneous graphs.}
On the one hand, most of the existing heterogeneous graph embedding methods  either insufficiently model the local structure under specific semantic, or neglect the heterogeneity when aggregating information from it.
{\color{blue}
On the other hand, representations from multiple semantics are not comprehensively integrated to obtain node embeddings with versatility.}
%
To address the problem, 
we propose a \textit{Heterogeneous Graph  Neural Network with Multi-View Representation Learning}~(named MV-HetGNN) 
for heterogeneous graph embedding by introducing the idea of multi-view representation learning.
The proposed model consists of view-specific ego graph encoding and auto multi-view fusion
to thoroughly learn complex structural and semantic information
for generating comprehensive and versatile node representations.
%
Extensive experiments on three real-world heterogeneous graph datasets show that the proposed MV-HetGNN model consistently outperforms all the state-of-the-art baselines in various downstream tasks, \eg node classification, node clustering, and link prediction.
\end{abstract} 
